CCAT-prime Collaboration: Science Goals and Forecasts with Prime-Cam on the Fred Young Submillimeter Telescope

We present a detailed overview of the science goals and predictions for the Prime-Cam direct detection camera/spectrometer being constructed by the CCAT-prime collaboration for dedicated use on the Fred Young Submillimeter Telescope (FYST). The FYST is a wide-field, 6-m aperture submillimeter telescope being built (first light in mid-2024) by an international consortium of institutions led by Cornell University and sited at more than 5600 meters on Cerro Chajnantor in northern Chile. Prime-Cam is one of two instruments planned for FYST and will provide unprecedented spectroscopic and broadband measurement capabilities to address important astrophysical questions ranging from Big Bang cosmology through reionization and the formation of the first galaxies to star formation within our own Milky Way galaxy. Prime-Cam on the FYST will have a mapping speed that is over ten times greater than existing and near-term facilities for high-redshift science and broadband polarimetric imaging at frequencies above 300 GHz. We describe details of the science program enabled by this system and our preliminary survey strategies.

==> highz_old.tex <==
Much of star formation (SF) is hidden from view in the optical bands due to dust in the molecular clouds that envelop the newly formed stars. 
This dust absorbs the starlight, heats up and re-radiates the power at far-infrared (FIR) wavelengths. 
This dust-enshrouded star formation is important over cosmic time --  the cosmic optical background (COB) power and cosmic infrared background (CIB) energy density are roughly equal \citep[e.g.,][]{Dole06,2013Burgarella}. 
Consequently, when considering the star formation history of the Universe, both optical and FIR wavelengths must be considered. 
A discrepancy in the expected infrared output, inferred from the dust masses in local galaxies, and the observed measurements of the CIB suggested first that IR sources must become more numerous at higher redshift and be a critical component of early mass build-up \citep[e.g.,][]{Lagache05}, which was further supported by studies of the most luminous ``submillimeter galaxies'' \citep[e.g.,][]{Casey2014}. 
\edit2{Subsequent \textit{Spitzer} and \textit{Herschel} surveys} resolved  $\sim\,$80\% of the CIB at $\lambda$$\,<\,$$160\,\mu$m %has been resolved 
into individual galaxies. %by \textit{Spitzer} and \textit{Herschel}, which provided 
\edit2{This work provided robust} constraints on the cosmic SF history at $z\lesssim1.5$\ and demonstrated that about $70\,\%$ was dust-enshrouded at these epochs \citep{2013Magnelli}. \edit2{However, the dust emission from higher redshift galaxies is redshifted to longer wavelength ($250$$\,>\mu$m) where the inability of the 3.5$\,$m \textit{Herschel} telescope to separate emission from multiple galaxies within a single spatial beam (source confusion) becomes a serious problem.  Therefore, at $z\gtrsim1.5$\, the }
%Despite this success, at $250$$\,<\,$$\lambda$$\,<\,$$500\,\mu$m, where the 3.5$\,$m \textit{Herschel} telescope was hampered by confusion (inability to separate emission from multiple galaxies within a single resolution element), 
fraction of CIB resolved into individual galaxies drops to only $\sim$10\%\ \citep{Bethermin12}.
Such limitation is unfortunate and critical, as in this wavelength range the CIB is dominated by $z\gtrsim1.5$ galaxies \citep{Bethermin12} while providing the best dust-obscured star formation rate proxy for this galaxy population (Figure~\ref{fig:SFH} {\it lower right}). 
Thus, to study the source of the CIB at $\lambda$$\,>\,$$160\,\mu$m in detail (understanding the physical properties of high-redshift galaxies contributing to the CIB), high-resolution IR surveys such as those done with \pcam on FYST need to be conducted.

\pcam on FYST provides the instrumentation and platform to enable studies of dusty star-forming galaxies (DSFGs) in the high-redshift and up to the early Universe.
With the 6\,m aperture of FYST, \pcam reaches about $3$ times deeper into the source confusion than was possible with the {\em Herschel} 3.5\,m telescope. 
Using the model of \citet{2017Bethermin}, we predict that confusion-limited \pcam surveys (DSS and CIB-Mid) will securely detect hundreds of thousands of galaxies at redshifts potentially as high as 6 (Fig.~\ref{fig:SFH}, {\it upper right}) and resolve into individual galaxies up to $\sim\,$40\% of the CIB at 850\,GHz. 
Its deep, yet wide-field ($100\,\deg^2$; e.g., CIB-mid) survey will sample environments on large scales that cannot be mapped with ALMA, and reach down to luminosities that remained inaccessible to {\em Herschel} (Fig.~\ref{fig:SFH}, {\it upper right}). 
The 850\,GHz band is critical to extract the infrared luminosities and subsequently the dust-obscured star formation rates to far greater precision than possible with long-wavelength surveys (e.g., LMT; Fig.~\ref{fig:SFH}, {\it lower right}) alone.
For example, the first followup of 350\,GHz-selected galaxies with {\em Herschel}-SPIRE at these high frequencies constrained the peak of their dust spectral energy distributions (SEDs) and allowed their dust temperatures and far-infrared luminosities to be measured for the first time, enabling accurate star formation rate constraints \citep{2010Chapman,2012Magnelli}. 
Today, measuring the peak of the dust SEDs is a prerequisite to precision constraints on dusty and highly star-forming galaxies at $1\gtrsim z\gtrsim6$, and putting them in context with the cosmic history of star formation \citep{2018Elbaz}.
Combining our surveys with synergistic work in the optical/near-infrared (DES, {\em{Rubin}}, {\em{Euclid}} and {\em{Roman}}) Prime-Cam will identify key parameters that regulate star formation (such as environment and matter content) over cosmic time of highly star-forming galaxies (SFR$\,\gtrsim 200\,M_{\odot}\,$yr$^{-1}$; Figure~\ref{fig:SFH} {\it upper right}). 
Such constraints are paramount to shed light on the formation of local massive ellipticals, likely produced from gas-rich mergers at high redshift that trigger violent and short-live star formation activities \citep{2006Hopkins,2007Faber}. 
Finally, thanks to its depth and wide coverage, \pcam surveys will statistically constrain through stacking the mean dust-obscured star formation rates of galaxy population not directly detected but selected from large optical/near-infrared surveys. 
Using this approach, it will be virtually possible to estimate the \textit{total} star formation activities of ``normal'' (i.e., $L\ast$) galaxies out to $z\sim5$ \citep[galaxies which have $L_{\rm IR}^{L_\ast} \sim 0.1 \times L_{\rm IR}^{\rm \pcam\ limit}$ at $z\sim1-5$;][]{2013Magnelli,2013Gruppioni,2020Gruppioni}, and obtain for the first time a robust determination of the cosmic star formation history. 
Section 5.1 describes the methods and additional constraints on the cosmic history of star formation made possible by Prime-Cam data, and in section 5.2 we present details of the surveys and delivered science results.

\subsection{Cosmic History of Star Formation}

The cosmic history of star formation, galaxy assembly, and matter content are encoded in the variation of the physical properties of galaxies with their spatial and redshift distributions \citep{2014Madau}. 
In order to properly trace and understand the formation and evolution of galaxies large statistical studies are required over representative cosmic volumes that adequately sample the entire range of cosmic environments (${>}$\,100\,$\deg^2$; Fig.~\ref{fig:SFH} {\it upper and lower left}).
Over the next decade, short-wavelength surveys will be carried out to commensurate depths and areas at X-ray to near-infrared wavelengths (e.g., \emph{eROSITA}, \emph{Rubin}, DES, \emph{Euclid}, and \emph{Roman}) tracing unobscured star formation. 
However, the dust-obscured half of star formation is only robustly accessible at rest-frame FIR wavelengths, which are redshifted into the $250{-}500\,\mu$m wavelength range where no commensurate survey capabilities exist yet. 
Since the properties of dust in galaxies appear to evolve significantly with cosmic time \citep{Casey14}, short-wavelength surveys have to rely on order-of-magnitude extinction corrections that are too large for measuring reliable SF properties. 
Without accurate measurements of FIR luminosities, the total (i.e., direct + obscured stellar light) star-formation rates and SF properties in galaxy evolution studies therefore remain out of reach.

At $1<z<6$, the 850\,GHz band of \pcam will probe the FIR emission of galaxies near the rest-frame of the dust emission SED peak, thereby providing an excellent proxy for estimating FIR luminosities and dust obscured star-formation rates in the high-redshift Universe  - typically 2 to 3 times more accurately than is possible with, for example, LMT/ALMA mm-wave surveys alone, and 3 - 5 times more accurately for galaxies also detected by \pcam lower frequency (down to 220 GHz) bands ($5{-}8\%$ according to the model of B\'ethermin et al. \citeyear{2017Bethermin}; Fig.~\ref{fig:SFH}, {\it lower right}).
\pcam therefore fills a critical gap with its unique combination of deep 850\,GHz coverage, significantly improved spatial resolution (${\sim}\,15$\,arcsec at 850\,GHz) compared to previous facilities operating at these frequencies \citep[in particular \emph{Herschel},][]{Lutz2014}, and a very large field-of-view ($0.78\,\deg^2$; ${>}\,200{,}000$ times larger than ALMA at 850\,GHz).
Through deep, large-area contiguous submillimeter wave surveys \citep[critically complementing ultra-deep ``pencil
beam'' surveys with ALMA;][]{Walter2016,Aravena2016,Dunlop2017,Franco2018,2019GonzalezLopez}, 
\pcam surveys will in its lifetime securely detect millions of star-forming galaxies across a broad range of cosmic environments out to $z\sim5$, probing typically about 3 times deeper than the most sensitive {\em Herschel} surveys \citep{Lutz2014}. 

From direct observations of the FIR spectral energy distribution peak, accurate dust-obscured SFRs, can be inferred for the vast majority of dusty, highly star-forming (SFR$\,\gtrsim 200\,M_{\odot}\,$yr$^{-1}$) galaxies out to $z\sim5$ within the wide-field optical/near-infrared survey fields that will become available at the time that construction of the telescope is completed \citep{parshley/2018a}. 
For about $5{-}10\%$ of these galaxies, detection in several \pcam lower frequency (down to 220 GHz) bands will be also available, that will yield accurate dust masses and temperatures.
Additional physical parameters of these massive and intensely star-forming systems may be determined for a subset of the sample by combining \pcam surveys with these synergistic optical/near-infrared surveys to obtain their photometric redshifts, stellar masses, and unobscured fractions of the SFR, which is ${\le}\,50$\,\% globally \citep{2013Burgarella,2015Pannella,2020Gruppioni}. The ability to obtain photometric redshifts from O/IR surveys will however depend on redshift and obscuration \citep{2003Chapman,2005Chapman,2012Casey,2017Danielson}, and far-infrared based photometric redshifts will need to be used for a substantial fraction of the sources, especially at higher redshfits. 
%
From this, it is then possible to statistically identify the key parameters regulating matter assembly (cosmic epoch verses environment) in these extreme systems which are likely the progenitors of local massive ellipticals.
\pcam wide-area surveys will particularly being advantageous in this context as it will allow for accurate measurement of the clustering properties of these extreme systems and thereby test their evolutionary link to today’s massive ellipticals which are known to reside in the central region of massive groups and clusters. 
Through stacking of hundreds of galaxies, \pcam will also statistically constrain the mean dust-obscured star formation rates of galaxy population not directly detected but selected from large optical/near-infrared surveys ($S/N^{\rm stack} \propto S/N^{ind.} \times \sqrt{N_{\rm stack}}$). 
From this, it is then possible to obtain a significantly improved determination of the cosmic star formation history. 
Finally, because of the large survey areas, it will also be possible to discover large samples of strongly-lensed dusty galaxies for detailed follow-up studies with ALMA and {\em{JWST}} \citep[e.g.,][]{canameras2015,Hodge2020} and IR-bright galaxy protoclusters at high redshift as signposts of early structure formation \citep{oteo18,Miller2018,2019GomezGuijarro,Hill2020}.

\pcam surveys will also be suitable to uncover very dusty sources (including the most intense starbursts in the Universe) that are entirely missed by even the deepest optical/near-infrared surveys, over a broad luminosity range; out to $z>7$ \citep[e.g.,][]{riechers13b,riechers17,Strandet2016,Brisbin2017,Marrone2018,Wang2019,Reuter2020}. 
These sources are very rare, and only very small numbers are currently known at $z>5$, due to the limited sensitivity, wavelength coverage, and/or areas of past and current (sub)millimeter surveys \citep[see ][for a recent overview]{riechers20a}.
While such sources are bright in mm-wave surveys, they can be discriminated from the dominant lower-redshift foreground with the inclusion of the shorter submillimeter wave band of \pcam \citep{riechers17}.
As illustrate in Figure~\ref{fig:SFH} ({\it upper right}), applying such a 850 GHz ``dropout'' technique will indeed be a powerful tool to select $z>4$ candidates.
By obtaining good statistics on this population of dusty, highly star-forming galaxies one can address important issues of galaxy evolution. For example: when and how did local ``red-and-dead'' ellipticals form? 
Two leading theories that link the evolutionary tracks are through major mergers, which trigger intense, yet short-lived starburst leaving behind a passively evolving elliptical, and massive star-forming galaxies that are starved of gas by a ``too-hot'' halo. 
Overall, in the \pcam galaxy evolution survey, through the detection of large samples of dusty, highly star-forming galaxies over a broad range of redshifts, the mechanism of evolution into local ellipticals can be studied in detail.

\begin{figure*}[t]
\begin{center}
\includegraphics[width=0.9\textwidth]{figures/SFH_v5.jpg}
\caption{Contiguous wide-area multi-wavelength \pcam surveys will measure the dust-obscured star formation properties of hundreds of thousands of galaxies out to $z\sim6$ with high precision. 
This will greatly enhance our picture of cosmic galaxy evolution, probing 2-to-3 times lower luminosities than \emph{Herschel}-SPIRE at $z>1$ (due to source confusion; see insets in {\it upper left} panel) while sampling large-scale environments (voids, average density regions, groups, and clusters) over 100 times larger areas than feasible to map with ALMA (the field of view of ALMA is a fraction of a single \pcam pixel) and providing more accurate dust-obscured star formation measurements than current or future millimeter-only surveys. 
{\it Upper left:} Sky coverage of the CIB-Mid survey (i.e., $\sim\,$100\,deg$^{2}$) compared to the dark matter distribution at $z\sim1.4$ from the Millennium simulation \citep{springel18}.
Insets illustrate how the improved angular resolution of \pcam helps going deeper into the source confusion than was possible with the {\em Herschel} 3.5\,m telescope. 
{\it Lower left:} Survey area needed to detect at least one halo of mass, $M_{\rm h}$, at a redshift, $z$, within a redshift bin, $\Delta z = 0.1\times z$, as inferred using the halo mass function of \citet{2013Murray}.
Different lines correspond to different halo masses. 
{\it Upper right:} Simulated \pcam survey luminosity limits, compared to surveys feasible with existing instrumentation covering the $250-500\,\mu$m wavelength range, which is critical to measure accurately the infrared luminosity of $1\lesssim z \lesssim 6$ galaxies. 
\pcam will probe up to $3\times$ deeper than \emph{Herschel}-SPIRE, while sampling environments and luminosities inaccessible to ALMA surveys because of sampling variance \citep[gray areas inferred using the model of][]{2017Bethermin}. 
{\it Lower right:} Predicted reliability (16th to 84th percentiles) of far-infrared luminosity measurements, highlighting the vast improvements with the \pcam $350\,\mu$m (850 GHz) band and wide spectral coverage. These reliabilities were inferred by fitting (or renormalizing) single modified blackbody function with $\beta=1.5$ and $T_{\rm dust}\in[20{-}50\,{\rm K}]$ \citep[e.g.][]{2012Magnelli} to the variety of SEDs from the \citet{2007Draine} template library. 
}
\label{fig:SFH}
\end{center}
\end{figure*}

\subsection{Dusty Star-Forming Galaxy Surveys}
\label{sec:DSFG}
In its early pilot phases, our DSFG survey will cover the rich, multi-wavelength GAMA fields (${\sim}\,100\,\deg^{2}$ total) to the confusion limit at $350\,\mu$m (Figure~\ref{fig:SFH}, {\it upper left inset}), making use of the best quartile in PWV. Ultra-deep integrations covering $4{-}16\,\deg^{2}$ over key galaxy evolution survey fields (COSMOS and E-CDFS) will also be obtained, in parallel alongside the EoR intensity mapping fields, and will reach far below the confusion limit, providing a precise measurement of the confusion noise on the scales most relevant to \pcam. The full survey will also cover the ${\sim}\,100\,\deg^{2}$ extended SDSS Stripe-82 area (previously covered only shallowly by \emph{Herschel}-SPIRE) to comparable depths. Overall, using the model of \citet{2017Bethermin}, we expect to detect $440{,}000$ individual galaxies above a signal-to-noise ratio of 5 within each of our confusion-limited ${\sim}\,100\,\deg^{2}$ survey (e.g., CIB-Mid), $1{,}300$ of which we expect to be at $z>5$ and detected primarily by the lower frequency Prime-Cam modules (220-410\,GHz).
We note that the $z>5$ far-infrared luminosity function is still highly uncertain \citep{casey18} %(Casey et al.\ 2018) % ApJ 862 77 
and a factor of $\approx$2 uncertainty exists on the number of $z>5$ sources that will be found in these surveys.
Figure~5 illustrates these model surveys and luminosity limits. The model includes those galaxies detected at a given band, so indeed the highest redshift galaxies constrained at 850\,GHz alone need to be detected at this frequency and  therefore have larger SFRs ($>1000$M$_\odot$/yr) as shown in the upper left panel. Including all the Prime-Cam bands, there are a much larger number of galaxies extending to lower luminosities, and the majority of these anticipated $z>5$ galaxies will be undetected dropouts at 850GHz. 

In summary, the large and comprehensive sample of dusty, star forming galaxies that will result from \pcam galaxy evolution survey will: (1) lead to robust constraints on the the luminosities of bright submillimeter sources from $z=1$ out to $z>5$, and accordingly to an improved constraint on the bright end of the luminosity function (i.e., $L_{\rm IR}\gtrsim 10 \times L_\ast$); (2) statistically constrain the cosmic star formation history out to $z\sim5$; (3) reveal the impact of environment the population of dusty, highly star-forming (SFR$\,\gtrsim 200\,M_{\odot}\,$yr$^{-1}$) galaxies and (4) reveal their evolutionary link to today's ellipticals; and (5) allow for the study of ``exotic'' sources, such as protoclusters and strongly lensed sources, extending luminosity limits downwards by about 3 times that achieved by {\it Herschel} at high ($z>3$) redshifts.

